Bootstrap Masked Visual Modeling via Hard Patches Mining

Masked visual modeling has attracted much attention due to its promising potential in learning generalizable representations. Typical approaches urge models to predict specific contents of masked tokens, which can be intuitively considered as teaching a student (the model) to solve given problems (predicting masked contents). Under such settings, the performance is highly correlated with mask strategies (the difficulty of provided problems). We argue that it is equally important for the model to stand in the shoes of a teacher to produce challenging problems by itself. Intuitively, patches with high values of reconstruction loss can be regarded as hard samples, and masking those hard patches naturally becomes a demanding reconstruction task. To empower the model as a teacher, we propose Hard Patches Mining (HPM), predicting patch-wise losses and subsequently determining where to mask. Technically, we introduce an auxiliary loss predictor, which is trained with a relative objective to prevent overfitting to exact loss values. Also, to gradually guide the training procedure, we propose an easy-to-hard mask strategy. Empirically, HPM brings significant improvements under both image and video benchmarks. Interestingly, solely incorporating the extra loss prediction objective leads to better representations, verifying the efficacy of determining where is hard to reconstruct. The code is available at https://github.com/Haochen-Wang409/HPM.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/6.ack.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


This work was supported in part by the Major Project for New Generation of AI (No.~2018AAA0100400), the National Natural Science Foundation of China (No.~61836014, No.~U21B2042, No.~62072457, No.~62006231), and the InnoHK program.


==> sections/8.bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/wanghaochen.jpg}}]{Haochen Wang}
is currently a Ph.D. student at the Center of Research on Intelligent Perception and Computing, State Key Laboratory of Multimodal Artificial Intelligence Systems, Institute of Automation, Chinese Academy of Sciences, under the supervision of Prof. Zhaoxiang Zhang.
%
Prior to that, he received his B.S. degree from Shanghai Jiao Tong University in 2022.
%
His research interests include label-efficient semantic segmentation, self-supervised visual representation learning, multi-modal learning, and vision foundation models.
%
He serves as the reviewer for several representative journals such as TMM and TNNLS, and top-level conferences like CVPR, ICCV, ICLR, and NeurIPS.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/fanjunsong.jpg}}]{Junsong Fan}
received his B.S. degree from the School of Automation Science and Electrical Engineering, Beihang University in 2016.
Then, he joined the Center of Research on Intelligent Perception and Computing, National Laboratory of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences, under the supervision of Prof. Zhaoxiang Zhang, and received his Ph.D. degree in 2022.
He is now an assistant professor in the Centre for Artificial Intelligence and Robotics, Hong Kong Institute of Science \& Innovation, Chinese Academy of Sciences.
His research interests include computer vision and machine learning, label-free learning, and visual perception in open worlds.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/WangYuxi}}]{Yuxi Wang}
%
received his B.S. degree from North Eastern University, China in 2016, and his Ph.D. degree from the University of Chinese Academy of Sciences, Institute of Automation, Chinese Academy of Sciences in January 2022.
He is now an assistant professor at the Center for Artificial Intelligence and Robotics, Hong Kong Institute of Science \& Innovation, Chinese Academy of Science. 
His research interests include transfer learning, domain adaptation, and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Author_KaiyouSong.eps}}]{Kaiyou Song}
%
received his B.S. degree from Wuhan University in 2015, and his Ph.D. degree from Huazhong University of Science and Technology, in 2021. 
%
He has been working as a researcher at MEGVII Technology since 2021. 
%
His current research interests include visual representation learning, visual understanding, and multimodal learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/tiancaiwang.png}}]{Tiancai Wang}
%
is currently a senior researcher at MEGVII Technology.
%
He obtained his M.S. degree from Tianjin University in 2020. 
%
Previously, he was an intern researcher at the Inception Institute of Artificial Intelligence and MEGVII Technology in 2018 and 2019, respectively. 
%
His current research interest includes autonomous driving, computer vision, and 3D perception. 
%
He has published more than thirty papers on some top conferences and journals, such as CVPR, ICCV, ECCV, and NeurIPS. 
%
He also serves as the reviewer for several high-impact AI conferences and journals.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/xiangyuzhang.jpg}}]{Xiangyu Zhang}
received his Ph.D. degree from Xi'an Jiaotong University in 2017, and currently is the leader of the Foundation Model team in MEGVII Research. 
%
His research interests mainly focus on deep learning models for practical vision tasks, especially efficient neural architecture design, AutoML/NAS, and CNN backbones for detection/segmentation/face tasks, etc. 
%
He has proposed a series of widely used CNN architectures and algorithms such as ResNets/ShuffleNets/RepVGG. 
%
He won the Best Paper Award in CVPR 2016. 
%
His total number of Google Scholar citations is over 270,000. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/zhangzhaoxiang.jpg}}]{Zhaoxiang Zhang}
received his B.S. degree in Circuits and Systems from the University of Science and Technology of China (USTC) in 2004 and his Ph.D. degree from the National Laboratory of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences in 2009. 
In October 2009, he joined the School of Computer Science and Engineering, Beihang University, as an Assistant Professor (2009-2011) and an Associate professor (2012-2015). 
In July 2015, he returned to the Institute of Automation, Chinese Academy of Sciences as a full Professor in the Center for Research on Intelligent Perception and Computing (CRIPAC) and the National Laboratory of Pattern Recognition (NLPR).
His research interests include Computer Vision, Pattern Recognition, and Machine Learning. Recently, he specifically focuses on biologically inspired intelligent computing and its applications in human analysis and scene understanding. 
He has published more than 200 papers in international journals and conferences, including reputable international journals such as IEEE TPAMI, IJCV, and JMLR, and top-level international conferences like CVPR, ICCV, ECCV, ICLR, NeurIPS, AAAI, and IJCAI. He served or is serving as the Associated Editor of IEEE TCSVT, Pattern Recognition, and Frontiers of Computer Science. He has served as the Area Chair of reputable international conferences like CVPR, ICCV, AAAI, IJCAI, ACM MM, ICPR, and ACCV.
\end{IEEEbiography}
